Accelerating SpMM Kernel with Cache-First Edge Sampling for Graph Neural Networks

Graph neural networks (GNNs), an emerging deep learning model class, can extract meaningful representations from highly expressive graph-structured data and are therefore gaining popularity for wider ranges of applications. However, current GNNs suffer from the poor performance of their sparse-dense matrix multiplication (SpMM) operator, even when using powerful GPUs. Our analysis shows that 95% of the inference time could be spent on SpMM when running popular GNN models on NVIDIA's advanced V100 GPU. Such SpMM performance bottleneck hinders GNNs' applicability to large-scale problems or the development of more sophisticated GNN models. To address this inference time bottleneck, we introduce ES-SpMM, a cache-first edge sampling mechanism and codesigned SpMM kernel. ES-SpMM uses edge sampling to downsize the graph to fit into GPU's shared memory. It thus reduces the computation cost and improves SpMM's cache locality. To evaluate ES-SpMM's performance, we integrated it with a popular GNN framework, DGL, and tested it using representative GNN models and datasets. Our results show that ES-SpMM outperforms the highly optimized cuSPARSE SpMM kernel by up to 4.35x with no accuracy loss and by 45.3x with less than a 1% accuracy loss.

==> sections/sec_4_2.tex <==
\section{CacheSample Implementation}
\label{sec:impl}

In this section, we describe the details of our \cachesample{} kernel implementation, and how we integrate CacheSample into a real system.

\subsection{Kernel Implementation}

\begin{algorithm}[t!]
    \caption{CacheSample SpMM Kernel Pseudo Code}
    \label{alg:cachesample}
    \begin{algorithmic}[1]
    \STATE {\bfseries Input:} \text{A.data, A.row\_ptr, A.col\_ind, B, shmem\_width}
    \STATE {\bfseries Output:} \text{C}
    \FOR{each thread}
    \STATE \_\_shared\_\_ sh\_data[], sh\_cols[];
    \STATE row\_id, col\_id, sh\_offset, row\_nnz = get\_offsets();
    \STATE S = min(row\_nnz, shmem\_width); 
    % \STATE \COMMENT{\textit{Step 1: Sample A and load up shared memory}}
    \FOR{$i \gets threadIdx$ \textbf{to} $S$ \textbf{step} $blockDim$}
    \STATE samp\_idx = cal\_sample\_index($i$, row\_nnz);
    \STATE sh\_data[i], sh\_cols[i] = load\_A(samp\_idx);
    \ENDFOR
    \STATE \_\_syncthreads();
    % \STATE \COMMENT{\textit{Step 2: A loop to compute an element of C}}
    \FOR{$j \gets 0$ \textbf{to} $S$}
    \STATE acc += sh\_data[j] $\ast$ B[sh\_cols[j], col\_id];
    \ENDFOR
    \STATE C[row\_id, col\_id] = acc;
    \ENDFOR
  \end{algorithmic}
\end{algorithm}

CacheSample kernel takes sparse matrix A stored in the compressed-sparse row (CSR) format.
CSR is the most common used compressed format for storing the graph adj matrix, and supported by most of the sparse libraries such as Scipy \cite{scipy}, Eigen \cite{eigenweb} and Ligra \cite{ligra} and GNN frameworks like DGL \cite{dgl} and PyTorch Geometric \cite{pyg}.
Being able to work directly with the CSR format allows us to easily hook the CacheSample kernel into existing frameworks, and avoid the expensive overhead on converting sparse formats.
Since we target to accelerate GNN's inference in this work, using other formats also makes it almost impossible to achieve our goal since the format transformation time might exceed the inference time itself.

We illustrate the kernel pseudo code of CacheSample in Algorithm \ref{alg:cachesample}, which follows the principles highlighted in Section \ref{subsec:designs}.
The kernel is implemented in CUDA and thus we use CUDA's terminology in the pseudo code.
The input of the kernel are A's data, row pointers and column indices which are the three standard components of the CSR format, matrix B, and $s$ which is the threshold value used in the sampling and is also the shared memory width.
The kernel will produce one output, which is the matrix C.
The whole Algorithm \ref{alg:cachesample} is parallelized to each GPU thread.

In the beginning of the kernel, it calculates the row and column id of the C element that the thread will need to output.
The id calculations are based on the number of threads and thread-blocks we create for the kernel, and how we assign workload among them.
It also calculates other offsets the kernel will use in the later steps, such as the base position of the row's first nnz, and the shared memory row offset.
In our CacheSample implementation, we follow the row-split spirit as \cite{merge-spmm, gespmm} and assign multiple number of threads for each row.
However, unlike \cite{merge-spmm, gespmm} use 32 threads for a row, which is the number of threads in a warp, we choose to use the number of columns of C, $N$, as the number of threads for computing the results for a row.
%threads unit for a row's computation.
The reason is because we will use the same group of threads to load up the shared memory for a row, and the width of the shared memory $s$ could be large as 512 or bigger.
If we only use 32 threads per row, we will need a few iterations to load up the shared memory, which may take a long time.
Since the number of columns of C in GNN's computation typically ranges from 32 to 128, it is a good amount of threads to make the load up of the shared memory fast with not too many threads waiting (the waiting case is that when the row nnz is smaller than $s$, part of the threads will have no items to load during the last iteration).
Also, this arrangement lets one thread compute one element of C, which makes the threads assignment simpler.
The simple threads assignment has benefits such as making kernel code more readable, since sometimes, a CUDA kernel could be difficult to understand due to a complex threads assignment.
With this scheme, for a thread block of our CacheSample implementation, the number of threads in the X dim matches the number of columns of C, and we set the number of threads in y dim to 4.
Therefore, for a thread block, it will handle the workload for 4 output rows. 
The shared memory size will be set to $2 \times (4 \times s)$, since we need space for holding both A's data and indices and they need equal space.
Base on these setting, we will create $ceil(M / 4)$ number of thread blocks, where $M$ equals to number of rows of adj matrix A.
% is in charged using the thread and block index passed in by the CUDA driver base on the how much threads and thread blocks we create for the SpMM workload.
% which is in charged by that thread based on the threadIdx values passed in by the CUDA driver.
% It will also calculate the offsets that will be used in the later loops.
% This part is similar to other general SpMM implementations \cite{gespmm, gale2020sparse}.
% In our implementation, each GPU thread is in charge of one element of output C.

The second part is to do the sampling and load up the shared memory, which is the core of the CacheSample kernel.
As we discussed in the previous paragraph, we assign each thread to handle the computation for one element of C.
In this case, the threads handle the same row elements of C share the non-zero elements of the same row in A.
Therefore, we use $N$ threads to do the sampling for a row of A's non-zeros and load the sampled values and indices to a row of the shared memory.
The sampling function in the line 14 of Algorithm \ref{alg:cachesample} will use one of the sampling strategies mentioned in the section \ref{subsec:sampling}, take the original index and row nnz, and output a sampled index, $s\_idx$ for each time.
After that, we can use the sampled index to fetch A's values and column indices from the global memory to shared memory.
Note here, if we use the \bucket{} sampling strategy, the memory loading to A will be coalesced because concurrent threads will load values stored continuously on the memory.
If we use \simrand{} sampling, the data loading to A will be less coalesced since \simrand{} will generate random-like indices across the range of the nnz of each row.
However, since we create a good amount of threads to load up the shared memory and typically the desired width, $s$, isn't very big, the latency of the data loading can be hidden and it's still efficient.

After the sampling is done and the shared memory is loaded, the third part is to do the multiplication and accumulation to compute the output element of C based on items we sample and stored on the shared memory.
This part we follow similar design principle as \cite{merge-spmm}, in which concurrent threads in a thread block will handle the data fetch and compute in the the row but in neighbor columns of C and will fetch neighbor data in the same row of B.
By using this arrangement, the concurrent threads will fetch neighbor data in the same row of B and make the global memory access of B coalesced, which is the key to achieve high performance GPU kernel.
The rest of the third part is that each thread will get the needed B's data base on a row of the sampled A's indices and values read from the shared memory, accumulate through the multiplication results, store the output C value back to the global memory and finish the SpMM computation.

\subsection{System Integration}
We integrate our CacheSample kernel with DGL, a popular GNN framework allowing users to develop various GNN models easily in Python.
As we mentioned in the previous sections, CacheSample works directly on the standard CSR format.
This allows CacheSample can be integrated into existing systems that already support CSR.
We choose DGL among multiple options mainly because it provides a clean separation between the front-end API and the back-end kernel function.
In DGL's back-end, it uses \textit{cusparseSpMM()} function provided in the cuSparse vendor library to implement their SpMM operator.
Our CacheSample kernel takes the same inputs as the \textit{cusparseSpMM()} function and returns output in exactly the same format.
By following the same interface, we can seamlessly replace the \textit{cusparseSpMM()} function with our CacheSample kernel in the back-end implementation of DGL.
% By following the same interface, we can seamlessly replace the \textit{cusparseSpMM()} function with our CacheSample kernel.

Since we only need to modify the back-end side of the DGL framework, we can reuse all the front-end APIs in DGL and require no changes in a user's Python script to run a GNN model with our CacheSample kernel.
In other words, users can easily get a boosted speed for their GNN models by installing our modified version of DGL 
%\footnote{Our code is open source and can be found at https://github.com/uwsampl/gnn\_benchmark}.
This also allows us can test the performance of our CacheSample kernel with different GNN models in a rapid development time.

==> sections/sec_5_2.tex <==
\section{Evaluation}
\label{sec:eval}

In this section, we would describe our evaluation methodology and provide extensive experimental results to show the effectiveness of our CacheSample kernel. 

\subsection{Experimental Setup}
% As we discussed in the section \ref{sec:eval}, 
To ease the development of evaluating \cachesample{} on real GNN models, we integrate our \cachesample{} kernel with one of the most popular GNN frameworks, DGL.
Therefore, we use DGL to implement the GNN models in our experiments.
We pick two representative GNN models, GCN \cite{gcn} and GraphSage \cite{graphsage}, and perform node classification to evaluate our CacheSample kernel.
For the GraphSage model, we use mean as the feature aggregator.
These models both use SpMM since the feature aggregation of GCN is just sum and the mean feature aggregator of GraphSage involves sum operation. 
Since CacheSample is used to speedup SpMM operator, experimenting on GCN and GraphSage can show how effective CacheSample is.
Also, GCN and GraphSage are widely adopted in many other GNNs \cite{cluster-gcn, jknet, as-gcn, fastgcn, deepgcns, graphsaint, gcnii}.
Therefore, being able to show speedup on GCN and GraphSage provides good potential to accelerate other models which are based on them.

% \input{tables/dataset}

We test GCN and GraphSage on four representative node classification datasets that are commonly used in the GNNs' literatures.
The four datasets are Pubmed, Ogb-Arxiv, Ogb-Proteins and Reddit.
Pubmed is a citation network for research papers in the medical domain.
Ogbn-Arxiv is also a citation network collected by Open Graph Benchmark (OGB) \cite{ogb}.
Ogbn-Proteins is a protein-protein-interaction network, also collected by OGB.
Reddit is a social network recording the posts and comments relationship for the popular online forum, Reddit.
A brief summary of each datasets can be found in Table \ref{tab:dataset}.

As we can see from Table \ref{tab:dataset}, each dataset represents a different scale.
Pubmed represents a small size of graph with less number of nodes and edges.
Ogbn-Arxiv represents a small to medium size of graph with moderate number of nodes and edges.
Ogbn-Proteins also represents a medium to large size of graph with moderate number of nodes, but has much more edges compared to Ogbn-Arxiv.
Reddit represents a large size of graph with large number of nodes and edges.
Evaluating on datasets with scales from small to large can help us understand the usage of our CacheSample kernel better.
We categorize Pubmed and Ogbn-Arxiv as small datasets and Ogbn-Proteins and Reddit as large datasets in the following section for simplicity.

Before we evaluate the impact on the accuracy of our CacheSample kernel, we first trained the GCN and GraphSage models on the four datasets in their original state for ten times and kept the model weights with the best test accuracy.
The model parameters we use and the best accuracy we achieve for each model and dataset are shown in the Table \ref{tab:model}.
After the models are trained, we will replace the \textit{cusparseSpMM()} function in the DGL back-end to our CacheSampel kernel, re-compile the DGL framework, and perform inference to measure the test accuracy and execution time.
The training and inference for all the models and datasets in our experiments are done on AWS EC2 p3.2xlarge instance and use one NVIDIA's V100 GPU with 16GB memory.

\input{tables/model}

\subsection{Sampling Rates}
\label{subsec:sample_rate}
Echo the results shown in the Figure \ref{fig:edge_sample}, sampling rate is an important factor that will affect the test accuracy.
Since the four datasets in our experiments are in different scales and the shared memory size we can utilize is fixed for each GPU, it will have a different sampling rates for each datasets under a certain shared memory width target ($s$).
To obtain the sampling rates, we simulate the CacheSample behavior in Python and calculate the equivalent results and the results are reported in the Table \ref{tab:sample_rate}.
Note that the two sampling strategies we proposed in the section \ref{subsec:sampling} will have the same sampling rate for a given $s$, since they will fetch the same amount but just different sets of A's values and indices to the shared memory

As we can see from the Table \ref{tab:sample_rate}, for medium to small datasets like Pubmed and Ogbn-Arxiv, a small $s$ value can hold most of the edges.
When using a larger $s$, it can actually hold all the edges on the shared memory.
However, for larger size graphs such as Ogbn-Proteins and Reddit, the sampling rates are much lower and $s$ value equals to 256 can only hold around 34\% of edges for both of the datasets.
Base on this sampling rates analysis, we expect CacheSample can achieve little to no accuracy drop for small graphs, but a more distinct loss on the accuracy for large graphs.

\input{tables/sample_rate}
\input{exp_fig}

\input{tables/best2}

\subsection{Accuracy and Speedup for Different $S$}
% The accuracy plots
We plot the accuracies of GCN and GraphSage using our CacheSample kernel under different $s$ and sampling strategies for each datasets in Figure \ref{fig:cs_acc_gcn} and \ref{fig:cs_acc_sage}.
Note that the accuracy here is the test accuracy at the inference time with a pretrained model.
Recall that the mapping between $s$ and sampling rate for each dataset can be found in \ref{tab:sample_rate}.

As shown in the Figure \ref{fig:cs_acc_gcn} and \ref{fig:cs_acc_sage}, we obtain expected results as the discussions in section \ref{subsec:sample_rate}.
For the small datasets, Pubmed and Ogbn-Arxiv, CacheSample only has small to no accuracy loss across different $s$ values for both sampling strategies.
For the GraphSage on Pubmed, CacheSample has no accuracy loss even with the smallest $s$.

For the large datasets, Ogbn-Proteins and Reddit, we see a larger accuracy drop when $s$ is small.
However, when we increase the $s$ value, the accuracy will raise since more edges are used.
As we can see in the Figure \ref{fig:exp_acc_speedup}, \fr{} can give a better accuracy than \buc{} on the large datasets especially when $s$ is small.
For the Ogbn-Proteins dataset, we discover that \buc{} has a bigger accuracy decrease to \fr{} compared to other datasets.
We suspect that it's because the average number of edges in Ogbn-Proteins's graph is pretty high, and the way that \buc{} sampling picks a continuous region of indices will lost too much information of the graph structure and let the models hard to predict correct classification results.
However, since \fr{} will select indices from a larger perspective, it shows much higher accuracies than \buc{} for the Ogbn-Proteins dataset.
As we use larger $s$ such as 64 or 128 or above, \fr{} can actually achieve a similar level of accuracy as the baseline.
For the Reddit dataset, the average number of edges is also high and is only slightly lower than the Ogbn-Proteins.
But since it's an easier dataset that both GCN and GraphSage can achieve pretty high baseline accuracy (above 94\%), the accuracy difference between \buc{} and \fr{} are not as much as the results of Ogbn-Proteins.

\subsection{Speedup}
Here we compare CacheSample kernel time with the default implementation in DGL, which calls to the \textit{cusparseSpMM()} function provided in the cuSPARSE library.
We will use \textit{cuSPARSE} to infer the SpMM implementation of cuSPARSE library in the rest of paper for simplicity.
The speedups of CacheSample for different models, datasets, sampling strategies and $s$ are plotted in Figure \ref{fig:cs_speedup_gcn} and \ref{fig:cs_speedup_sage}.
We use PyTorch profiler to get the kernel time, and each speedup number is the average from ten times of inference.

We also see different speedup results between small and large datasets.
For the small datasets, CacheSample achieves more stable speedups from 2x to 4x across the $s$ values.
For the large datasets, we see a much higher range of speedup from 2x all the way up to 96x depends on how small $s$ is.
The reason for the different speedup ranges is because for the small datasets, the inference time is already fast in our baseline, which are 3ms to 20ms, and the space for speedup is limited.
However, due to less computation and better locality, CacheSample is still able to push the already fast runtime to the next level.
Note that at here, since the sampling rates for the small datasets are pretty high even with a small $s$, the speedup mostly comes from the locality improvement.

When we look at the speedups for the large datasets, we can see \buc{} constantly gives a higher speedup than \fr{}.
This shows that the sampling strategy plays a vital roles of the performance when there are more edges to be sampled.
Although \fr{} achieves a lower speedup than \buc{}, it still shows significant speedups compared to the cuSparse baseline.
Consider that \fr{} causes a smaller accuracy loss than \buc{}, \fr{} is a better sampling strategy to use to obtain good accuracy and speedup.
However, for a easier dataset such as Reddit, we can use \buc{} to achieve a faster inference time and can still have a good accuracy.

\subsection{Experiments Summary}
To show the effectiveness of our CacheSample more clearerly, we summarize the best speedup of CacheSample with less than 1\% accuracy loss for both of the models and all the datasets in the Table \ref{tab:best}.
As we can see from the Table \ref{tab:best}, CacheSample is able to achieve \textbf{25x} speedup compared to cuSparse for GCN on the Reddit dataset with only \textbf{0.96\%} accuracy drop when using \buc{} sampling strategy.
For GraphSage, CacheSample is able to achieve \textbf{4.35x} speedup with \textbf{no accuracy loss} on the Pubmed dataset.
When running GraphSage on Reddit dataset, our CacheSample kernel can achieve \textbf{45.3x} and \textbf{26.87x} speedup with only \textbf{0.92\%} and \textbf{0.76\%} accuracy loss when using \buc{} and \fr{} respectively.
Our experiments show that CacheSample can effectively speedup the representative GNN models's inference time among different scales of datasets.
% talk about the two sampling.


==> tables/breakdown.tex <==
\begin{table}[tb!]
\caption{\chien{change to a staked chart.}End-to-end compute time breakdown of the GCN model on different datasets. The time is measured in millisecond.}
\label{tab:breakdown}
% \vskip 0.15in
\begin{center}
\begin{small}
\begin{sc}
\scalebox{0.95}{
\begin{tabular}{l|rrr|r}
\toprule
Dataset & GEMM	& SpMM	& Other	 & SpMM Ratio \\
\midrule
Pubmed   & 0.32	& 0.68   & 3.28	& 15.94\% \\
Ogbn-Arxiv    & 6.32	& 14.01  & 4.39	& 56.67\% \\
Ogbn-Proteins & 4.23	& 173.20 & 4.12	& \textbf{95.40\%} \\
Reddit   & 5.81	& 99.86	 & 2.76	& \textbf{92.10\%} \\
\bottomrule
\end{tabular}}
\end{sc}
\end{small}
\end{center}
% \vskip -0.1in
\end{table}


